Coded Alternating Least Squares for Straggler Mitigation in Distributed Recommendations

Matrix factorization is an important representation learning algorithm, e.g., recommender systems, where a large matrix can be factorized into the product of two low dimensional matrices termed as latent representations. This paper investigates the problem of matrix factorization in distributed computing systems with stragglers, those compute nodes that are slow to return computation results. A computation procedure, called coded Alternative Least Square (ALS), is proposed for mitigating the effect of stragglers in such systems. The coded ALS algorithm iteratively computes two low dimensional latent matrices by solving various linear equations, with the Entangled Polynomial Code (EPC) as a building block. We theoretically characterize the maximum number of stragglers that the algorithm can tolerate (or the recovery threshold) in relation to the redundancy of coding (or the code rate). In addition, we theoretically show the computation complexity for the coded ALS algorithm and conduct numerical experiments to validate our design.

==> 4-Analysis.tex <==
\section{Algorithm Analysis}

In this section, we will divide the whole process into encoding, decoding, computation and communication 4 parts to analyse the work each worker or master should do. All the time of these 4 parts can be measured according to times of element-wise multiplication in matrix multiplication. For the matrix multiplication program $C=AB$, with $A\in\mathbb R^{m\times d}$ and $B\in\mathbb R^{d\times n}$, we assume the computation time as $\sum\limits_i^{mnd}T_{u(l)}$, where $T_{u(l)}\sim(\mu_u, \sigma_u)$ such that the expected computation time for the matrix multiplication computation time is proportional to the size of the matrix.

\subsection{Redundancy Analysis}
\begin{theorem}
\upshape{(Straggler resistance)} We use $K$ to represent the least number of workers it require to recover the result, then the relation between the storage load $\mu$ and number of workers $W$ can be represented as
\begin{IEEEeqnarray}{rcl}
K=\frac{W}{\mu}+ \sqrt{\frac{W}{\mu}}-1 \quad \mu>1
\label{fr:storageRedundancy}
\end{IEEEeqnarray}
where $W\geq h^2$.
\end{theorem}
\textit{Proof:} 
Suppose each worker have a same size of data partitions of $\tilde R$ with $k$ elements.
According to \eqref{partition:D} and the fact that each worker holds one partition of $R$, and there are $h^2$ partitions in $R$, and the number of elements in $R$ is $h^2k$.
So that $\mu$ could be represented as
\begin{IEEEeqnarray}{rcl}
\mu=\frac{Wk}{h^2k}=\frac{W}{h^2}
\label{fr:storagerate}
\end{IEEEeqnarray}


From Lemma \ref{lm:threshold}, we know the relation between $K$ and $h$. By replacing $h$ in \eqref{fr:recoverythreshold} by \eqref{fr:storagerate}, we can get \eqref{fr:storageRedundancy}.


\subsection{Computation Time}
\begin{theorem}
(Complexity Analysis)
For the whole process proposed in this algorithm depicted in Fig.\ref{fig:wholeprocess}, where we use $T$ to represent the number of iterations, and $n$ to represent the number of columns and rows of $B$\footnote{Here we assume that $n<m$ for R}. The complexity for each stage of the algorithm can be represented as the following form:

\begin{enumerate}
    \item\label{th:complexity:computation} The computation complexity can be represented as  $O(\frac{Tn^2d}{h^2})$ in each worker.
    
    \item\label{th:complexity:encoding} The encoding complexity, which denotes the complexity to do the encoding procedure denoted as $f_L$ and $f_R$ taken place in the master, is $O(\frac{TndW}{h})$. 
    
    \item\label{th:complexity:decoding} The decoding complexity, donotes the decoding procedure happened in the master, is $O(nd(h^2+h))$
\end{enumerate}


\end{theorem}

\textit{Proof:} 
For the computation time in workers  \ref{th:complexity:computation}),
According to \eqref{fr:est_T}, we know that the estimated running time of this algorithm. 
$n$ is the largest factor of influence of this algorithm, so that the second term in \eqref{fr:est_T} can be ignored. 
On the other hand, from \eqref{fr:floor_Phi} and \eqref{fr:ceil_Phi}, we know the $\Phi^{-1}(\cdot)$ is bounded. Then the first term plays a more important role in \eqref{fr:est_T}. Then the computation complexity in each worker could be represented as $O(\frac{Tn^2d}{h^2})$ for the whole algorithm in each worker.

For the encoding procedure in \ref{th:complexity:encoding}), depicted in black thick solid line, we noticed that there are 3 such types of encoding procedures in Fig.\ref{fig:wholeprocess}.
And the matrix to be encoded like $B$ and $E$ all share the same size, so we only need to consider one encoding procedure. The shape of one partition of  $B$ or $E$ is $\frac{nd}{h}$. So the complexity to compute the weighted sum is $\frac{TWnd}{h}$.

For the decoding procedure in \ref{th:complexity:decoding}), 
We know that there are 3 decoding steps in the whole algorithm, which has been marked in the Fig.\ref{fig:wholeprocess}. For the 3 EPC decoding procedure, the decoding complexity could be represented as $O(hSK)$, where $S$ represents the size of matrix multiplication result from each worker. Thus for decoding procedure 1, the decoding complexity is $O(Th(\frac{nd}{h})(h^2+h-1))$.
For decoding procedure in 2,3, the decoding complexity is $O(Td^2 (2h-1))$. Finally for the MDS decoding procedure, the decoding complexity is $O(T\frac{nd}{h}h)$. $n$ has the greatest impact in these terms. So the final complexity could be expressed as $O(Tnd(h^2+h))$.
 







\begin{lemma}
\label{pr:time_decrease}
In worker's computation stage, when doing the multiplication of matrices,
the computation time $T_{cp}$ decreases as $h$ grows.
\end{lemma}
\textit{Proof}: See Appendix \ref{ap:decrease}

\begin{remark}
$\mu$ and $\sigma$ are determined by the performance of the computer, which is hard to measure in this setup. When $\sigma$ is smaller, that is, each worker has a relatively stable time to process the same size of data, the order statistics would be close to each other, and therefore their influence become less important. Therefore, with larger $h$, each worker has smaller data to process, the total computation time could be less.

However, $n$ is always a large number in \eqref{fr:request}, so that this inequality always holds.
\end{remark}




\begin{proposition}
\upshape{(Select the number of partitions)}
In the proposed algorithm, to get a better partition method, in common configurations, e.g., when $W<100$. When $h^*=\lfloor \sqrt{W+\frac{3}{4}-s} \rfloor$, we will
achieve a relatively less expected computation time $\mathbb E[T_{cp}]$ when workers doing their computation task.

\end{proposition}

\textit{Proof}: 
According to the definition of stragglers
\begin{IEEEeqnarray}{rcl}
s+K\leq W
\label{fr:upperbound}
\end{IEEEeqnarray}

There are 4 decoding procedure in the algorithm, shown in figure \ref{fig:wholeprocess}, the recovery threshold for the first step to get  $E$ is the largest which is 
\begin{IEEEeqnarray}{rcl}
K=f_K(h)=h^2+h-1
\label{fr:threshold}
\end{IEEEeqnarray}



In \textbf{lemma} \ref{pr:time_decrease}, we have proved that the computation time $T_{cp}$ decreases as $h$ grows.
Therefore, to get smaller $T_{cp}$, we need to make $h$ greater.

It's easly known that $f_K(h)$ monotonously increased when $h\geq 1$, which is upper bounded by \eqref{fr:upperbound}.
Therefore, \eqref{fr:upperbound} and \eqref{fr:threshold} can be written as
\begin{IEEEeqnarray}{rcl}
h^2+h+s-(w+1)\leq 0
\end{IEEEeqnarray}
and therefore the best $h^*$ is got to make to make the computation time less.


\begin{remark}
Given $s$ and $W$, this proposition can help us find a number of partitions that will bring a shorter time in the computation procedure of workers, which will therefore save a large amount of time in practical.
\end{remark}



\subsection{Redundancy and resistance to Stragglers}






